A Holistic Framework for Analyzing the COVID-19 Vaccine Debate

The Covid-19 pandemic has led to infodemic of low quality information leading to poor health decisions. Combating the outcomes of this infodemic is not only a question of identifying false claims, but also reasoning about the decisions individuals make. In this work we propose a holistic analysis framework connecting stance and reason analysis, and fine-grained entity level moral sentiment analysis. We study how to model the dependencies between the different level of analysis and incorporate human insights into the learning process. Experiments show that our framework provides reliable predictions even in the low-supervision settings.

==> 6_qualitative.tex <==
\section{Qualitative Evaluation}

Characterizing the discussion around one or two events.

%\subsection{Extracting Events and Event-Centric Tweets}

%A website (https://www.ajmc.com/view/a-timeline-of-covid-19-vaccine-developments-in-2021) which contains a timeline of covid-19 events was scraped using beautiful soup. The following information was collected from the website: date of the event, title of the event, description of the event, and all hyperlinks that are present in the description. A natural language processing library - spacy was then used on the both the title and the description for Named Entity Extraction (NER). The duplicate entities were removed. For each entity extracted, it was mapped to the closest Wikipedia article using the Wikipedia API and that was used as a canonical entity. 

%The twitter academic API was used to extract all tweets that contained the words "covid vaccine" or "vaccine" from the months of January 2021 to September 2021. This information was stored alongside all of the relevant meta-data of the tweet. NER (alongside mapping the entity extracted to the closest Wikipedia article to be used as a canonical entity) with duplication removal was then performed on each of these tweets and the results were stored alongside the tweet ID, creation date of the tweet, and the tweet description.

%For each event, we went over all the tweets that were posted $\pm$n days (where n = 3) of the event and compared the entities of the event with the tweet. Each event has its own unique file with the tweets that matched its entities sorted from most matches to least matches.
